A Discrete de Rham method for linear and nonlinear fourth-order plate models

We develop and analyze a Discrete de Rham (DDR) method for the Kirchhoff--Love plate problem on general polygonal meshes and demonstrate its extension to geometrically nonlinear plates. The construction uses local degrees of freedom and polynomial reconstructions, avoiding the implementation difficulties associated with globally $C^1$-conforming approximation spaces. A new deflection reconstruction obtained from the discrete Hessian permits a uniform treatment of the load term at all polynomial degrees. The use of this reconstruction improves the convergence rates of previous DDR methods and enables the formulation of a lowest-order scheme with only vertex unknowns. We provide a stability and convergence analysis of the method and validate the theoretical results through a comprehensive set of numerical tests. The method is then extended to the coupled von K\'arm\'an equations, for which we demonstrate convergence numerically. We also study the flat-branch spectrum of a compressed perforated plate and its small-amplitude forced nonlinear response near the first critical load.

==> figures/von_karman_convergence_test/combined/unit-square-quad_airy_energy_norm_plot.tex <==
% Generated paper panel: one mesh family, all polynomial degrees.
\noindent\begin{tikzpicture}
\begin{loglogaxis}[
  width=\linewidth, height=0.78\linewidth,
  title={airy energy norm vs. $h$},
  xmin=0.022097086912169481, xmax=0.35355339059421481, enlarge x limits=0.07,
  ymin=2.2636079185545102e-05, ymax=15.842559146403262, enlarge y limits=false,
  xlabel={$h$}, title style={font=\small}, label style={font=\scriptsize},
  tick label style={font=\scriptsize}, grid=major,
  major grid style={gray!40},
  legend pos=south east, legend style={font=\scriptsize, inner sep=2pt}, legend cell align={left}
]
\addplot[color=blue, mark=*, solid, thick, mark options={solid, fill=blue, draw=blue}] coordinates { (3.5355339059421481e-1,6.5860968246306371e0) (1.7677669529722873e-1,3.2834971989775235e0) (8.8388347648650084e-2,1.6538540636839254e0) (4.4194173824334396e-2,8.3193545308540151e-1) (2.2097086912169481e-2,4.1725878079059636e-1) };
\addlegendentry{$k=0$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,6.5860968246306371e0) -- (axis cs:1.7677669529722873e-1,3.2834971989775235e0) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {1.00};
\draw[draw=none] (axis cs:1.7677669529722873e-1,3.2834971989775235e0) -- (axis cs:8.8388347648650084e-2,1.6538540636839254e0) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.99};
\draw[draw=none] (axis cs:8.8388347648650084e-2,1.6538540636839254e0) -- (axis cs:4.4194173824334396e-2,8.3193545308540151e-1) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.99};
\draw[draw=none] (axis cs:4.4194173824334396e-2,8.3193545308540151e-1) -- (axis cs:2.2097086912169481e-2,4.1725878079059636e-1) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {1.00};


\addplot[color=red, mark=square*, solid, thick, mark options={solid, fill=red, draw=red}] coordinates { (3.5355339059421481e-1,6.0266532959624652e-1) (1.7677669529722873e-1,1.0210516037308744e-1) (8.8388347648650084e-2,1.4613748696680673e-2) (4.4194173824334396e-2,1.9232922943043847e-3) (2.2097086912169481e-2,2.4565737718440739e-4) };
\addlegendentry{$k=1$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,6.0266532959624652e-1) -- (axis cs:1.7677669529722873e-1,1.0210516037308744e-1) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.56};
\draw[draw=none] (axis cs:1.7677669529722873e-1,1.0210516037308744e-1) -- (axis cs:8.8388347648650084e-2,1.4613748696680673e-2) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.80};
\draw[draw=none] (axis cs:8.8388347648650084e-2,1.4613748696680673e-2) -- (axis cs:4.4194173824334396e-2,1.9232922943043847e-3) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.93};
\draw[draw=none] (axis cs:4.4194173824334396e-2,1.9232922943043847e-3) -- (axis cs:2.2097086912169481e-2,2.4565737718440739e-4) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.97};


\addplot[color=brown, mark=o, solid, thick, mark options={solid, fill=white, draw=brown}] coordinates { (3.5355339059421481e-1,2.0970813226016310e-1) (1.7677669529722873e-1,2.7386588170746070e-2) (8.8388347648650084e-2,3.4599340671064870e-3) (4.4194173824334396e-2,4.3458076335744524e-4) (2.2097086912169481e-2,5.4450068513801100e-5) };
\addlegendentry{$k=2$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,2.0970813226016310e-1) -- (axis cs:1.7677669529722873e-1,2.7386588170746070e-2) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.94};
\draw[draw=none] (axis cs:1.7677669529722873e-1,2.7386588170746070e-2) -- (axis cs:8.8388347648650084e-2,3.4599340671064870e-3) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.98};
\draw[draw=none] (axis cs:8.8388347648650084e-2,3.4599340671064870e-3) -- (axis cs:4.4194173824334396e-2,4.3458076335744524e-4) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.99};
\draw[draw=none] (axis cs:4.4194173824334396e-2,4.3458076335744524e-4) -- (axis cs:2.2097086912169481e-2,5.4450068513801100e-5) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.00};
\end{loglogaxis}
\end{tikzpicture}


==> figures/von_karman_convergence_test/combined/unit-square-quad_deflection_energy_norm_plot.tex <==
% Generated paper panel: one mesh family, all polynomial degrees.
\noindent\begin{tikzpicture}
\begin{loglogaxis}[
  width=\linewidth, height=0.78\linewidth,
  title={deflection energy norm vs. $h$},
  xmin=0.022097086912169481, xmax=0.35355339059421481, enlarge x limits=0.07,
  ymin=3.8249380763222699e-08, ymax=0.07686997024964079, enlarge y limits=false,
  xlabel={$h$}, title style={font=\small}, label style={font=\scriptsize},
  tick label style={font=\scriptsize}, grid=major,
  major grid style={gray!40},
  legend pos=south east, legend style={font=\scriptsize, inner sep=2pt}, legend cell align={left}
]
\addplot[color=blue, mark=*, solid, thick, mark options={solid, fill=blue, draw=blue}] coordinates { (3.5355339059421481e-1,2.9832034118235342e-2) (1.7677669529722873e-1,1.4876009738373851e-2) (8.8388347648650084e-2,7.5758497140978416e-3) (4.4194173824334396e-2,3.8349744574818876e-3) (2.2097086912169481e-2,1.9290696680466428e-3) };
\addlegendentry{$k=0$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,2.9832034118235342e-2) -- (axis cs:1.7677669529722873e-1,1.4876009738373851e-2) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {1.00};
\draw[draw=none] (axis cs:1.7677669529722873e-1,1.4876009738373851e-2) -- (axis cs:8.8388347648650084e-2,7.5758497140978416e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.97};
\draw[draw=none] (axis cs:8.8388347648650084e-2,7.5758497140978416e-3) -- (axis cs:4.4194173824334396e-2,3.8349744574818876e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.98};
\draw[draw=none] (axis cs:4.4194173824334396e-2,3.8349744574818876e-3) -- (axis cs:2.2097086912169481e-2,1.9290696680466428e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.99};


\addplot[color=red, mark=square*, solid, thick, mark options={solid, fill=red, draw=red}] coordinates { (3.5355339059421481e-1,2.0149749459855695e-3) (1.7677669529722873e-1,4.4859783306093525e-4) (8.8388347648650084e-2,7.4750910733603266e-5) (4.4194173824334396e-2,1.0654661676570235e-5) (2.2097086912169481e-2,1.4177998634139281e-6) };
\addlegendentry{$k=1$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,2.0149749459855695e-3) -- (axis cs:1.7677669529722873e-1,4.4859783306093525e-4) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.17};
\draw[draw=none] (axis cs:1.7677669529722873e-1,4.4859783306093525e-4) -- (axis cs:8.8388347648650084e-2,7.4750910733603266e-5) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.59};
\draw[draw=none] (axis cs:8.8388347648650084e-2,7.4750910733603266e-5) -- (axis cs:4.4194173824334396e-2,1.0654661676570235e-5) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.81};
\draw[draw=none] (axis cs:4.4194173824334396e-2,1.0654661676570235e-5) -- (axis cs:2.2097086912169481e-2,1.4177998634139281e-6) node[pos=0.50, above, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.91};


\addplot[color=brown, mark=o, solid, thick, mark options={solid, fill=white, draw=brown}] coordinates { (3.5355339059421481e-1,6.2116091322997758e-4) (1.7677669529722873e-1,6.5330211396489723e-5) (8.8388347648650084e-2,6.8637166783387503e-6) (4.4194173824334396e-2,8.0032085050280143e-7) (2.2097086912169481e-2,9.8559446187373673e-8) };
\addlegendentry{$k=2$}
\draw[draw=none] (axis cs:3.5355339059421481e-1,6.2116091322997758e-4) -- (axis cs:1.7677669529722873e-1,6.5330211396489723e-5) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.25};
\draw[draw=none] (axis cs:1.7677669529722873e-1,6.5330211396489723e-5) -- (axis cs:8.8388347648650084e-2,6.8637166783387503e-6) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.25};
\draw[draw=none] (axis cs:8.8388347648650084e-2,6.8637166783387503e-6) -- (axis cs:4.4194173824334396e-2,8.0032085050280143e-7) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.10};
\draw[draw=none] (axis cs:4.4194173824334396e-2,8.0032085050280143e-7) -- (axis cs:2.2097086912169481e-2,9.8559446187373673e-8) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.02};
\end{loglogaxis}
\end{tikzpicture}


==> figures/von_karman_convergence_test/combined/unit-square-tria_airy_energy_norm_plot.tex <==
% Generated paper panel: one mesh family, all polynomial degrees.
\noindent\begin{tikzpicture}
\begin{loglogaxis}[
  width=\linewidth, height=0.78\linewidth,
  title={airy energy norm vs. $h$},
  xmin=0.033145630368119572, xmax=0.53033008588991082, enlarge x limits=0.07,
  ymin=0.0001015902250616291, ymax=7.7306375691508142, enlarge y limits=false,
  xlabel={$h$}, title style={font=\small}, label style={font=\scriptsize},
  tick label style={font=\scriptsize}, grid=major,
  major grid style={gray!40},
  legend pos=south east, legend style={font=\scriptsize, inner sep=2pt}, legend cell align={left}
]
\addplot[color=blue, mark=*, solid, thick, mark options={solid, fill=blue, draw=blue}] coordinates { (5.3033008588991082e-1,3.5692185366408848e0) (2.6516504294495546e-1,1.7954998785409328e0) (1.3258252147247773e-1,9.2666926031981456e-1) (6.6291260736238949e-2,4.7638209873500886e-1) (3.3145630368119572e-2,2.4209545051496059e-1) };
\addlegendentry{$k=0$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,3.5692185366408848e0) -- (axis cs:2.6516504294495546e-1,1.7954998785409328e0) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.99};
\draw[draw=none] (axis cs:2.6516504294495546e-1,1.7954998785409328e0) -- (axis cs:1.3258252147247773e-1,9.2666926031981456e-1) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.95};
\draw[draw=none] (axis cs:1.3258252147247773e-1,9.2666926031981456e-1) -- (axis cs:6.6291260736238949e-2,4.7638209873500886e-1) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.96};
\draw[draw=none] (axis cs:6.6291260736238949e-2,4.7638209873500886e-1) -- (axis cs:3.3145630368119572e-2,2.4209545051496059e-1) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.98};


\addplot[color=red, mark=square*, solid, thick, mark options={solid, fill=red, draw=red}] coordinates { (5.3033008588991082e-1,3.7142020609309307e0) (2.6516504294495546e-1,1.0892674308058528e0) (1.3258252147247773e-1,2.0561686814664157e-1) (6.6291260736238949e-2,3.5768127995199704e-2) (3.3145630368119572e-2,5.8935453326482458e-3) };
\addlegendentry{$k=1$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,3.7142020609309307e0) -- (axis cs:2.6516504294495546e-1,1.0892674308058528e0) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {1.77};
\draw[draw=none] (axis cs:2.6516504294495546e-1,1.0892674308058528e0) -- (axis cs:1.3258252147247773e-1,2.0561686814664157e-1) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.41};
\draw[draw=none] (axis cs:1.3258252147247773e-1,2.0561686814664157e-1) -- (axis cs:6.6291260736238949e-2,3.5768127995199704e-2) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.52};
\draw[draw=none] (axis cs:6.6291260736238949e-2,3.5768127995199704e-2) -- (axis cs:3.3145630368119572e-2,5.8935453326482458e-3) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.60};


\addplot[color=brown, mark=o, solid, thick, mark options={solid, fill=white, draw=brown}] coordinates { (5.3033008588991082e-1,7.8033768118426006e-1) (2.6516504294495546e-1,8.6184564661871216e-2) (1.3258252147247773e-1,1.2738257795272363e-2) (6.6291260736238949e-2,1.6643457994976541e-3) (3.3145630368119572e-2,2.1144708813259177e-4) };
\addlegendentry{$k=2$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,7.8033768118426006e-1) -- (axis cs:2.6516504294495546e-1,8.6184564661871216e-2) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.18};
\draw[draw=none] (axis cs:2.6516504294495546e-1,8.6184564661871216e-2) -- (axis cs:1.3258252147247773e-1,1.2738257795272363e-2) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.76};
\draw[draw=none] (axis cs:1.3258252147247773e-1,1.2738257795272363e-2) -- (axis cs:6.6291260736238949e-2,1.6643457994976541e-3) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.94};
\draw[draw=none] (axis cs:6.6291260736238949e-2,1.6643457994976541e-3) -- (axis cs:3.3145630368119572e-2,2.1144708813259177e-4) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.98};
\end{loglogaxis}
\end{tikzpicture}


==> figures/von_karman_convergence_test/combined/unit-square-tria_deflection_energy_norm_plot.tex <==
% Generated paper panel: one mesh family, all polynomial degrees.
\noindent\begin{tikzpicture}
\begin{loglogaxis}[
  width=\linewidth, height=0.78\linewidth,
  title={deflection energy norm vs. $h$},
  xmin=0.033145630368119572, xmax=0.53033008588991082, enlarge x limits=0.07,
  ymin=3.9594507504983304e-07, ymax=0.038943907611352038, enlarge y limits=false,
  xlabel={$h$}, title style={font=\small}, label style={font=\scriptsize},
  tick label style={font=\scriptsize}, grid=major,
  major grid style={gray!40},
  legend pos=south east, legend style={font=\scriptsize, inner sep=2pt}, legend cell align={left}
]
\addplot[color=blue, mark=*, solid, thick, mark options={solid, fill=blue, draw=blue}] coordinates { (5.3033008588991082e-1,1.8400170029678489e-2) (2.6516504294495546e-1,9.9353044537560265e-3) (1.3258252147247773e-1,5.3216694162443344e-3) (6.6291260736238949e-2,2.7583995650417030e-3) (3.3145630368119572e-2,1.4059310993653400e-3) };
\addlegendentry{$k=0$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,1.8400170029678489e-2) -- (axis cs:2.6516504294495546e-1,9.9353044537560265e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.89};
\draw[draw=none] (axis cs:2.6516504294495546e-1,9.9353044537560265e-3) -- (axis cs:1.3258252147247773e-1,5.3216694162443344e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.90};
\draw[draw=none] (axis cs:1.3258252147247773e-1,5.3216694162443344e-3) -- (axis cs:6.6291260736238949e-2,2.7583995650417030e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.95};
\draw[draw=none] (axis cs:6.6291260736238949e-2,2.7583995650417030e-3) -- (axis cs:3.3145630368119572e-2,1.4059310993653400e-3) node[pos=0.35, above, text=blue, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {0.97};


\addplot[color=red, mark=square*, solid, thick, mark options={solid, fill=red, draw=red}] coordinates { (5.3033008588991082e-1,1.5683851692940672e-2) (2.6516504294495546e-1,3.6569743678952693e-3) (1.3258252147247773e-1,7.2523561887058972e-4) (6.6291260736238949e-2,1.2776160366623809e-4) (3.3145630368119572e-2,2.1601641376227165e-5) };
\addlegendentry{$k=1$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,1.5683851692940672e-2) -- (axis cs:2.6516504294495546e-1,3.6569743678952693e-3) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.10};
\draw[draw=none] (axis cs:2.6516504294495546e-1,3.6569743678952693e-3) -- (axis cs:1.3258252147247773e-1,7.2523561887058972e-4) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.33};
\draw[draw=none] (axis cs:1.3258252147247773e-1,7.2523561887058972e-4) -- (axis cs:6.6291260736238949e-2,1.2776160366623809e-4) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.50};
\draw[draw=none] (axis cs:6.6291260736238949e-2,1.2776160366623809e-4) -- (axis cs:3.3145630368119572e-2,2.1601641376227165e-5) node[pos=0.50, below, text=red, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {2.56};


\addplot[color=brown, mark=o, solid, thick, mark options={solid, fill=white, draw=brown}] coordinates { (5.3033008588991082e-1,1.0454028586064396e-3) (2.6516504294495546e-1,4.5838484741369102e-4) (1.3258252147247773e-1,5.5212766020863344e-5) (6.6291260736238949e-2,6.7162767737451441e-6) (3.3145630368119572e-2,8.3801662685939743e-7) };
\addlegendentry{$k=2$}
\draw[draw=none] (axis cs:5.3033008588991082e-1,1.0454028586064396e-3) -- (axis cs:2.6516504294495546e-1,4.5838484741369102e-4) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {1.19};
\draw[draw=none] (axis cs:2.6516504294495546e-1,4.5838484741369102e-4) -- (axis cs:1.3258252147247773e-1,5.5212766020863344e-5) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.05};
\draw[draw=none] (axis cs:1.3258252147247773e-1,5.5212766020863344e-5) -- (axis cs:6.6291260736238949e-2,6.7162767737451441e-6) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.04};
\draw[draw=none] (axis cs:6.6291260736238949e-2,6.7162767737451441e-6) -- (axis cs:3.3145630368119572e-2,8.3801662685939743e-7) node[pos=0.65, above, text=brown, fill=white, fill opacity=0.8, text opacity=1, inner sep=1pt, font=\scriptsize] {3.00};
\end{loglogaxis}
\end{tikzpicture}

